Upside and Downside Risk Exposures of Currency Carry Trades via Tail Dependence

Currency carry trade is the investment strategy that involves selling low interest rate currencies in order to purchase higher interest rate currencies, thus profiting from the interest rate differentials. This is a well known financial puzzle to explain, since assuming foreign exchange risk is uninhibited and the markets have rational risk-neutral investors, then one would not expect profits from such strategies. That is, according to uncovered interest rate parity (UIP), changes in the related exchange rates should offset the potential to profit from such interest rate differentials. However, it has been shown empirically, that investors can earn profits on average by borrowing in a country with a lower interest rate, exchanging for foreign currency, and investing in a foreign country with a higher interest rate, whilst allowing for any losses from exchanging back to their domestic currency at maturity. This paper explores the financial risk that trading strategies seeking to exploit a violation of the UIP condition are exposed to with respect to multivariate tail dependence present in both the funding and investment currency baskets. It will outline in what contexts these portfolio risk exposures will benefit accumulated portfolio returns and under what conditions such tail exposures will reduce portfolio returns.

==> (Matthew_Ames)_Innovations_in_Risk_Management/CopulaModels_GWP_26_Feb_2014_v1_0_0.tex <==
\section{Generalised Archimedean Copula Models for Currency Exchange Rate Baskets}

As noted in the previous section we develop flexible mixture Archimedean copula models for the currency baskets. Such models have the advantage that they produce asymmetric dependence relationships in the upper tails and the lower tails in the multivariate model.
In addition we can perform a type of model selection purely by incorporating into the estimation the mixture weights associated with each dependence hypothesis obtained from each mixture component. We consider three models; two Archimedean mixture models and one outer power transformed Clayton copula. The mixture models considered are the Clayton-Gumbel mixture and the Clayton-Frank-Gumbel mixture, where the Frank component allows for periods of no tail dependence within the basket as well as negative dependence. We fit these copula models to each of the long and short baskets separately. 

\begin{definition}[Mixture Copula] 
A mixture copula is a linear weighted combination of copulae of the form:
\begin{equation}
C_M(\mathbf{u}; \mathbf{\theta}) = \sum_{i=1}^N w_i C_i ({\bf u};{\bf \theta_i}) 		%% CHANGE TO \Theta
\end{equation}
where  $0 \leq w_i \leq 1 \;\; \forall i \in \{1, ..., N\}$ and $\sum_{i=1}^N w_i = 1$
\end{definition}

Thus we can combine a copula with lower tail dependence, a copula with positive or negative dependence and a copula with upper tail dependence to produce a more flexible copula capable of modelling the multivariate log returns of forward exchange rates of a basket of currencies. 

%Since we consider Archimedean copula mixture components, we next recall the definition of the generator. A function $\psi$ is said to generate an Archimedean copula if it satisfies the properties in Definition \ref{archm_gen}.

% Archimedean generator
\begin{definition}[Archimedean Generator]
An Archimedean generator is a continuous, decreasing function $\psi:[0, \infty) \rightarrow [0, 1]$ which satisfies the following conditions:
\begin{enumerate}
\item $\psi(0) = 1$,
\item $\psi(\infty) = lim_{t \rightarrow \infty} \psi(t) = 0$,
\item $\psi$ is strictly decreasing on $[0, inf\{t: \psi(t) = 0\}]$
\end{enumerate}
\label{archm_gen}
\end{definition}

\begin{definition}[Archimedean Copula]
A d-dimensional copula C is called Archim- edean if it can be represented as:
\begin{equation}
C({\bf u}) = \psi \{\psi^{-1}(u_1) + \cdots + \psi^{-1}(u_d)\} = \psi \{t({\bf u}) \} \;\;\;\; \forall {\bf u} \in [0, 1]^d
\label{eq:archimedean_copula}
\end{equation}
where $\psi$ is an Archimedean generator and $\psi ^{-1}:[0, 1] \rightarrow [0, \infty)$ is the inverse generator with $\psi^{-1}(0) = inf\{t: \psi(t) = 0\}$.
\end{definition}

One can then obtain formulas for computing the copula densities, of relevance to parameter estimation under a maximum likelihood approach. We can see from Equation~(\ref{eq:density}) that we are required to compute high dimensional derivatives of a composite function. In order to achieve this we utilise a specific multivariate chain rule result widely known as the Fa\`{a} di Bruno's Formula, see \cite{faa1857note} and discussions in for example \cite{constantine1996multivariate} and \cite{roman1980formula}. 

\begin{definition}[Archimedean Copula Density]
\cite{mcneil2009} prove that an Archimedean copula C admits a density c if and only if $\psi^{(d-1)}$ exists and is absolutely continuous on $(0, \infty)$. When this condition is satisfied, the copula density c is given by
\begin{equation}
c({\bf u})\;\; = \;\; \frac{ \partial^d C(u_1, \ldots , u_d)}{\partial u_1 \ldots \partial u_d} \;\;
= \;\;\ \psi^{(d)} \{t({\bf u})\} \prod_{j=1}^d (\psi^{-1})'(u_j) \;\; , \;\;\;\; {\bf u} \in (0, 1)^d
\label{eq:density}
\end{equation}
\end{definition}





==> (Matthew_Ames)_Innovations_in_Risk_Management/DataDescriptionBasketFormation_GWP_27_Feb_2014_v1_0_0.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Exchange Rate Multivariate Data Description and Currency Portfolio Construction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In our study we fit copula models to the high interest rate basket and the low interest rate basket updated for each day in the period 02/01/1989 to 29/01/2014 using log return forward exchange rates at one month maturities for data covering both the previous 6 months and previous year as a sliding window analysis on each trading day in this period. 

%Next we discuss briefly the marginal MLE estimations for l.g.g.d. and GARCH(1,1) models.

Our empirical analysis consists of daily exchange rate data for a set of 34 currency exchange rates relative to the USD, as in \cite{Menkhoff2012}. The currencies analysed included: Australia (AUD), Brazil (BRL), Canada (CAD), Croatia (HRK), Cyprus (CYP), Czech Republic (CZK), Egypt (EGP), Euro area (EUR), Greece (GRD), Hungary (HUF), Iceland (ISK), India (INR), Indonesia (IDR), Israel (ILS), Japan (JPY), Malaysia (MYR), Mexico (MXN), New Zealand (NZD), Norway (NOK), Philippines (PHP), Poland (PLN), Russia (RUB), Singapore (SGD), Slovakia (SKK), Slovenia (SIT), South Africa (ZAR), South Korea (KRW), Sweden (SEK), Switzerland (CHF), Taiwan (TWD), Thailand (THB), Turkey (TRY), Ukraine (UAH) and the United Kingdom (GBP).

We have considered daily settlement prices for each currency exchange rate as well as the daily settlement price for the associated 1 month forward contract. We utilise the same dataset (albeit starting in 1989 rather than 1983 and running up until January 2014) as studied in \cite{Lustig2011} and \cite{Menkhoff2012} in order to replicate their portfolio returns without tail dependence risk adjustments. Due to differing market closing days, e.g. national holidays, there was missing data for a couple of currencies and for a small number of days. For missing prices, the previous day's closing prices were retained. 

As was demonstrated in Equation (\ref{UIP}), the differential of interest rates between two countries can be estimated through the ratio of the forward contract price and the spot price, see \cite{Juhl2006} who show this holds empirically on a daily basis. Accordingly, instead of considering the differential of risk free rates between the reference and the foreign countries, we build our respective baskets of currencies with respect to the ratio of the forward and the spot prices for each currency. On a daily basis we compute this ratio for each of the $n$ currencies (available in the dataset on that day) and then build five baskets. The first basket gathers the $n/5$ currencies with the highest positive differential of interest rate with the US dollar.
These currencies are thus representing the ``investment" currencies, through which we invest the money to benefit from the currency carry trade. The last basket will gather the $n/5$ currencies with the highest negative differential (or at least the lowest differential) of interest rate.
These currencies are thus representing the ``financing" currencies, through which we borrow the money to build the currency carry trade.

Given this classification we investigate then the joint distribution of each group of currencies to understand the impact of the currency carry trade, embodied by the differential of interest rates, on currencies returns. In our analysis we concentrate on the high interest rate basket (investment currencies) and the low interest rate basket (funding currencies), since typically when implementing a carry trade strategy one would go short the low interest rate basket and go long the high interest rate basket.




==> (Matthew_Ames)_Innovations_in_Risk_Management/Discussion_MA_14_Nov_2013_v3_0_0.tex <==
\section{Conclusion}
\label{conclusion}

In this paper, we have shown that the positive and negative multivariate tail risk exposures present in currency carry trade baskets are additional factors needing careful consideration when one constructs a carry portfolio. Ignoring these exposures leads to a perceived risk return profile that is not reflective of the true nature of such a strategy.
In terms of marginal model selection, it was shown that one is indifferent between the log Generalised Gamma model and the frequently used GARCH(1,1) model. However, in combination with the three different Archimedean copula models considered in this paper the log Generalised Gamma marginals provided a better overall model fit.





%
%This article sheds light on an important topic that has been discussed in the recent financial literature which is the Uncovered interest rate parity (UIP) puzzle. This market phenomenon is particularly interesting from a theoretical standpoint as well as for the understanding of financial market mechanisms. It has been demonstrated that the currency markets were indeed not respecting empirically a fundamental relation in finance which connects the currency exchange rates and the interest rates associated with two different countries. The main contribution of this article has been to propose a rigorous statistical modelling approach which captures the specific statistical features of both the individual currency log-return distributions as well as the joint features such as the dependence structures prevailing between all the exchange rates. This has helped to understand a previously unexplored stochastic feature of the UIP violation.
%
%In achieving this goal, we first assessed the marginal statistical features of each of the 34 currencies on an assumed locally stationary sliding window of six months, over all the trading days in the period 02/01/1989 to 29/01/2014. 
%This showed that the flexible l.g.g.d. model was capable of capturing a range of skew-kurtosis relationships present in the real data.
%
%%We found that a simple LogNormal marginal distribution would not produce a suitable statistical fit for some of the key currencies that are regularly present in the high interest rate basket throughout this period. As detailed in the results section this was notably the case in unstable economies such as developing countries (for instance Turkey, Brazil or South Africa) where political stability or default risk create sudden and violent adjustments to their currency exchange rates with other countries. 
%
%%We note that these currencies are still of direct significance to currency carry trade strategies since according to the modern portfolio theory this intrinsic risk borne by an investor in these currencies can be diversified and mitigated by adding to the considered portfolio other currencies which depend themselves on different sources of intrinsic risk. This would effectively establish a diversified portfolio of currencies violating the UIP hypothesis and would thus provide a very attractive average return for a very limited risk which has been the conclusion of several recent empirical studies in the finance literature. 
%
%%The conclusion of this is that we cannot exclude these currencies from our high interest rate basket analysis, even though they may demonstrate attributes resulting primarily from significant changes in their countries' political and financial structures. As a result we needed to obtain more flexible marginal models to capture the features of these currencies more adequately. Consequently we modelled each currency exchange rate return marginally via a flexible three parameter parametric model which offers a wide range of skew-kurtosis relationships as well as the possibility of light exponential tails and heavier sub-exponential tail behaviours such as the LogNormal member. The parametric family of distributions we selected for this purpose was the log-generalized gamma distribution. 
%
%Having modelled the marginal attributes of the high and low interest rate currency baskets over time adequately, it was then our main emphasis to assess the multivariate dependence features of the currency baskets. In particular how this may change over time within a given basket, where we were particularly interested in the effect of the composition of the basket over time, and the response of the multivariate dependence features of the modelled basket and how it may respond in periods of heightened market volatility versus more stable periods. In addition to this within basket temporal analysis, from the perspective of undertaking a currency carry trade strategy, we would need to consider the relative relationships between the temporal dependence features of the high interest rate and low interest rate currency baskets. 
%We demonstrate several interesting features from our model fits relating to asymmetries between the high and low interest rate baskets over time, especially during periods of high volatility in global markets. One way we ascertained such periods was through a graphical comparison of the VIX versus features of the multivariate dependence relationships we modelled. Importantly we found substantial evidence to support arguments for time varying behaviours both in the structural dependence hypotheses posed about the currency baskets, as captured by the relevant contributing copula components to the multivariate mixture model. As well as substantial evidence for significant tail dependence features in both the high and low interest rate baskets, which again displayed interesting asymmetries between the high and low interest rate baskets over time. 
%
%The financial interpretation of the significance of these findings is related to the fact that it demonstrates that historically average rewards from a currency carry trade portfolio can be exposed to a significant risk of large losses arising from joint adverse movements in the currencies that would typically comprise the high and low interest rate baskets that an investor would go long and short when performing a currency carry trade. Hence, we conclude that our second contribution to the literature has been to rigorously demonstrate that such assertions relating to the profitability of the currency carry trade are failing to appropriately take into consideration an important component of the risk which characterizes these types of portfolios of currencies named carry trade portfolios, i.e. the upper and lower tail dependence features that we show are empirically present consistently in historic data.
%
%We conclude that indeed the copula theory we employed allows us to demonstrate statistically that beyond the intrinsic risk associated to high interest rate countries (which are generally paying higher interest rates to compensate for a higher risk) typically studied in the literature from a marginal perspective, another source of risk plays an important role. This second source of risk is related to the dependence structures linking these high interest rate currencies, more specifically the significant tail dependence features observed in our model analysis. We indeed proved through a mixture of Archimedean copulae the significant presence of tail dependence among high interest rate currencies which could have dramatic consequences on the carry trade portfolio's risk profile when accounted for appropriately in risk reward analysis. As a matter of fact, the tail dependence directly influences the diversity of the assets and thus reduces the appealing convergence property stated by the modern portfolio theory. 
%
%Said differently, our copula based probabilistic modelling approach allows us to demonstrate that besides the intrinsic risk associated to each particular high interest rate currency, another factor constitutes a determining source of risk which turns out to be the level of risk aversion prevailing in the market. It was demonstrated in our analysis that both upper and lower tail dependence features displayed significant association and asymmetries with each other between the high and low interest rate baskets during periods of relative financial stability versus periods of heightened market volatility.
%
%These tail dependence features in the high interest rate basket were significantly increasing during crisis periods leading to an increased exposure associated with utilising such currency baskets (which were no longer diversified due to the presence of significant tail dependence features) in a carry trade. That being said, a rational portfolio manager's natural risk aversion tells them that they should receive an additional remuneration in order to offset any additional sources of risk associated to an investment. Therefore, to properly assess the profitability of the currency carry trade, such tail dependence features should be incorporated into the analysis of the risk-reward. To conclude, our paper rigorously tempers the too often claimed attractiveness of the currency carry trade and provides to investors a risk management tool in order to control and monitor the risk contained in such positions.
%


==> (Matthew_Ames)_Innovations_in_Risk_Management/FittingtheModels_GWP_26_Feb_2014_v1_0_0.tex <==
%\section{Likelihood Based Estimation of the Mixture Copula Models}

%% WHY IS THIS BEFORE THE section heading ???


%In the following section we consider two stages to estimate the multivariate basket returns, firstly the estimation of suitable heavy tailed marginal models for the currency exchange rates (relative to USD), followed by the estimation of the dependence structure of the multivariate model composed of multiple exchange rates in currency baskets for long and short positions. To achieve this we consider a copula model framework where we utilise the well-known result of Sklar's theorem (see \cite{Nelsen2006}) as it allows one to separate the multivariate distribution into its marginal distributions and the dependence structure between the margins known as a copula distribution, which is unique for continuous marginal models.
%
%This result demonstrates how copula models therefore provide a mechanism to model the marginal behaviour of each currency and then separately to focus on developing hypotheses regarding the possible dependence structures between the log returns of the forward exchange rates of the currencies in the baskets, which can be tested through parametrization of a model via a copula and then a process of model selection.
%




%\section{Two Stage Estimation: Inference Function For the Margins}
\section{Currency Basket Model Estimations via Inference Function For the Margins}
\label{section:likelihood}

% MOVED HERE 27 Feb 2014 MATT
The inference function for margins (IFM) technique introduced in \cite{Joe1996} provides a computationally faster method for estimating parameters than Full Maximum Likelihood, i.e. simultaneously maximising all model parameters and produces in many cases a more stable likelihood estimation procedure. 
This two stage estimation procedure was studied with regard to the asymptotic relative efficiency compared with maximum likelihood estimation in \cite{Joe2005} and in \cite{Hafner2010}. It can be shown that the IFM estimator is consistent under weak regularity conditions.
%An alternative approach to copula model parameter estimation that is popular in the literature is known as the Maximum Partial Likelihood Estimator (MPLE) detailed in \cite{genest1995semiparametric}.


% However, it is not fully efficient for the copula parameters. Nevertheless, it is widely used for its ease of implementation and efficiency in large data settings such as the models we consider in this study.



%We begin this section with a discussion on the choices we make for the marginal distributions for each of the currencies specified in the baskets constructed for the high interest rate currencies and also the baskets for the low interest rate currencies.

In modelling parametrically the marginal features of the log return forward exchange rates, we wanted flexibility to capture a broad range of skew-kurtosis relationships as well as potential for sub-exponential heavy tailed features. In addition, we wished to keep the models to a selection which is efficient to perform inference and easily interpretable. We consider a flexible three parameter model for the marginal distributions given by the Log-Generalized-Gamma distribution (l.g.g.d.), see details in \cite{lawless1980inference}, where
%therefore considered a first analysis utilizing LogNormal distributions for the monthly forward exchange rate returns, which would be equivalent to specification of a Normality assumption on the distribution for the log return forward exchange rates. This model is given by the following parametric density, for a random variable $X \sim F(x;\mu,\sigma)$, in Equation \ref{EqnLN} below.
%\begin{equation} \label{EqnLN}
%f_X(x;\mu,\sigma) = \frac{1}{x\sqrt{2\pi\sigma^2}}\exp\left( -\frac{\left(\ln x - \mu\right)^2}{2\sigma^2} \right)
%\end{equation}
%with the shape parameter $\sigma^2 > 0$ and the log-scale parameter $\mu \in \mathbb{R}$ and the support $x \in (0,\infty)$.
%We found when analysing the goodness-of-fit for this LogNormal model on each of the assets in the 49 currencies considered, over both 6 month and 1 year sliding windows, that the fit of the LogNormal model would be systematically rejected as a suitable model for a couple of currencies. In the majority of cases over these sliding windows (locally stationary time series) the LogNormal model was more than adequate. However, since some of the currencies that were rejecting this fit were appearing regularly in the high interest rate baskets we also decided to consider
%
%a flexible three parameter model for the marginal distributions given by the Log-Generalized-Gamma distribution (l.g.g.d.), see details in \cite{lawless1980inference} and \cite{consul1971log}.
%The l.g.g.d. is a parametric model based on the generalized gamma distribution which is highly utilized in lifetime modelling and survival analysis. 
$Y$ has a l.g.g.d. if $Y = \mbox{log} (X)$ such that $X$ has a g.g.d. The density of $Y$ is given by
%The log transformed g.g.d. random variable $Y = \ln X$ is given by the density % of the l.g.g.d. in Equation \ref{EqnLGGD}.
\begin{equation} \label{EqnLGGD}
f_{Y}(y; k,u,b) = \frac{1}{b \Gamma(k)}\exp\left[k\left(\frac{y - u}{b} \right) - \exp\left(\frac{y-u}{b}\right) \right],
\end{equation}
with $u = \mbox{log} \, (\alpha)$, $b = \beta^{-1}$ and the support of the l.g.g.d. distribution is $y \in \mathbb{R}$.

This flexible three parameter model admits
%is particularly interesting in the context of the marginal modelling we are considering because many well-used distributions in the modelling of currency exchange rates are special cases. 
the LogNormal model as a limiting case (as $k \rightarrow \infty$). In addition the g.g.d. also includes the exponential model $(\beta=k=1)$, the Weibull distribution $(k=1)$ and the Gamma distribution $(\beta=1)$.

%Next we discuss how one can perform inference for the multivariate currency basket models using these marginal models and the mixture copula discussed previously.

As an alternative to the l.g.g.d. model we also consider a time series approach to modelling the marginals,given by the GARCH($p$,$q$) model, as described in \cite{bollerslev1986generalized} and \cite{brechmann2012risk}, and characterised by the error variance:

\begin{equation}
\sigma^2 = \alpha_0 + \sum\limits_{i=1}^q \alpha_i \epsilon_{t-i}^2 + \sum\limits_{i=1}^p \beta_i \sigma_{t-i}^2 \;\; .
\end{equation}


%\subsection{Two Stage Estimation: Inference Function For the Margins}

%The inference function for margins (IFM) technique introduced in \cite{Joe1996} provides a computationally faster method for estimating parameters than Full Maximum Likelihood, i.e. simultaneously maximising all model parameters and produces in many cases a more stable likelihood estimation procedure. 
%An alternative approach to copula model parameter estimation that is popular in the literature is known as the Maximum Partial Likelihood Estimator (MPLE) detailed in \cite{genest1995semiparametric}.
%
%The procedure we adopt for likelihood based estimation is the two stage estimation known as Inference function for the Margins which is studied with regard to the asymptotic relative efficiency of the two-stage estimation
%procedure compared with maximum likelihood estimation in \cite{Joe2005} and in \cite{Hafner2010}. It can be shown that the IFM estimator is consistent under weak regularity conditions. However, it is not fully efficient for the copula parameters. Nevertheless, it is widely used for its ease of implementation and efficiency in large data settings such as the models we consider in this study.

%In our study we fit copula models to the high interest rate basket and the low interest rate basket updated for each day in the period 02/01/1989 to 29/01/2014 using log return forward exchange rates at one month maturities for data covering both the previous 6 months and previous year as a sliding window analysis on each trading day in this period. Next we discuss briefly the marginal MLE estimations for l.g.g.d. and GARCH(1,1) models.

% MarginsX
\subsection{Stage 1: Fitting the Marginal Distributions via MLE}

%In the first step we fit the marginal distributions to the l.g.g.d. model.
% In the case of the LogNormal model this is achieved effortlessly since we may utilise the well-known analytic expressions for the MLE estimates:
%\begin{equation}
%\begin{split}
%\hat\mu_j &= \frac{1}{N}\sum_j \log\left(x_j\right) \\
%\hat\sigma_j &=  \sqrt{\frac{1}{N}\sum_j \log\left(x_j\right)^2 - \hat\mu_j^2}
%\end{split}
%\end{equation}
The estimation for the three model parameters in the l.g.g.d. can be challenging due to the fact that a wide range of model parameters, especially for $k$, can produce similar resulting density shapes (see discussions in \cite{lawless1980inference}). To overcome this complication and to make the estimation efficient it is proposed to utilise a combination of profile likelihood methods over a grid of values for $k$ and perform profile likelihood based MLE estimation for each value of $k$, over the other two parameters $b$ and $u$. The differentiation of the profile likelihood for a given value of $k$ produces the system of two equations:
\begin{equation}
%\begin{split}
\exp(\tilde\mu) = \left[ \frac{1}{n}\sum_{i=1}^n \exp\left(\frac{y_i}{\tilde\sigma\sqrt{k}}\right) \right]^{\tilde\sigma \sqrt{k}}\\
\hspace{5mm} ; \hspace{5mm}
\frac{\sum_{i=1}^n y_i \exp\left(\frac{y_i}{\tilde\sigma\sqrt{k}}\right)}{\sum_{i=1}^n \exp\left(\frac{y_i}{\tilde\sigma\sqrt{k}}\right)} - \overline{y} - \frac{\tilde\sigma}{\sqrt{k}} = 0 \; ,
%\end{split}
\label{lggd_mle}
\end{equation}
where $n$ is the number of observations, $y_i = \mbox{log} \, x_i$, $\tilde\sigma = b/\sqrt{k}$ and $\tilde\mu = u + b \, \mbox{log} \,k$. The second equation is solved directly via a simple root search to give an estimation for $\tilde{\sigma}$ and then substitution into the first equation results in an estimate for $\tilde{\mu}$. Note, for each value of $k$ we select in the grid, we get the pair of parameter estimates $\tilde\mu$ and $\tilde\sigma$, which can then be plugged back into the profile likelihood to make it purely a function of $k$, with the estimator for $k$ then selected as the one with the maximum likelihood score.
As a comparison we also fit the GARCH(1,1) model using the MATLAB MFEtoolbox using the default settings.

\subsection{Stage 2: Fitting the Mixture Copula via MLE}

In order to fit the copula model the parameters are estimated using maximum likelihood on the data after conditioning on the selected marginal distribution models and their corresponding estimated parameters obtained in Stage 1. These models are utilised to transform the data using the CDF function with the l.g.g.d. MLE parameters ($\hat k$, $\hat u$ and $\hat b$) or using the conditional variances to obtain standardised residuals for the GARCH model. Therefore, in this second stage of MLE estimation we aim to estimate either the one parameter mixture of CFG components with parameters ${\bf\underline\theta} = (\rho_{clayton}, \rho_{frank}, \rho_{gumbel}, \lambda_{clayton}, \lambda_{frank}, \lambda_{gumbel})$, the one parameter mixture of CG components with parameters ${\bf\underline\theta} = (\rho_{clayton}, \rho_{gumbel}, \lambda_{clayton}, \lambda_{gumbel})$  or the two parameter outer power transformed Clayton with parameters ${\bf\underline\theta} = (\rho_{clayton}, \beta_{clayton})$. 
%This is achieved in each case by the conditional maximum likelihood. This involves maximising 
The log likelihood expression for the mixture copula models, is given generically by:
\begin{equation}
l({\bf\underline\theta}) = \sum_{i=1}^n \mbox{log} \; c(F_1(X_{i1};\hat\mu_1, \hat\sigma_1), \dots, F_d(X_{id};\hat\mu_d, \hat\sigma_d))  \; + \; \sum_{i=1}^n \sum_{j=1}^d \mbox{log}  \;f_j(X_{ij};\hat\mu_j, \hat\sigma_j).
\label{loglik}
\end{equation}

%For example in the case of the Clayton-Frank-Gumbel mixture copula we need to maximise on the log-scale the following expression.
%\begin{equation}
%\begin{aligned}
%l({\bf\underline\theta}) = \sum_{i=1}^n log \; \big\lbrack & \lambda_C * \left(c_{\rho_C}^C \left(F_1 \left(X_{i1};\hat\mu_1, \hat\sigma_1 \right) \dots, F_d \left(X_{id};\hat\mu_d, \hat\sigma_d \right)\right) \right)  \\ 
%&+ \lambda_F* \left(c_{\rho_F}^F \left(F_1 \left(X_{i1};\hat\mu_1, \hat\sigma_1 \right) \dots, F_d \left(X_{id};\hat\mu_d, \hat\sigma_d \right)\right) \right)  \\ 
%&+ \lambda_G* \left(c_{\rho_G}^G \left(F_1 \left(X_{i1};\hat\mu_1, \hat\sigma_1 \right) \dots, F_d \left(X_{id};\hat\mu_d, \hat\sigma_d \right)\right) \right) \big\rbrack
%%\; + \; \sum_{i=1}^n \sum_{j=1}^2 log  \;f_j(X_{ij};\hat\mu_i, \hat\sigma_i)
%\end{aligned}
%\label{cgloglik}
%\end{equation}

This optimization is achieved via a gradient descent iterative algorithm which was found to be quite robust given the likelihood surfaces considered in these models with the real data. Alternative estimation procedures such as expectation-maximisation were not found to be required.

%To illustrate this point, at this stage it is instructive to present some examples of the shapes of the profile likelihoods that are being optimized over for some of the important copula model parameters in the CFG mixture example for a 6 month window of data randomly selected from the data set for both the high interest rate basket and the low interest rate basket. 

%Example plots of the profile likelihood for the 5-dimensional optimisation space for two different example days can be seen in Figures~\ref{profile_like_plot1} and~\ref{profile_like_plot2}.


%\begin{remark}
%A number of randomly selected copula fits from across the time period were analysed. The profile likelihood plots showed level sets which were not particularly complicated or multi-modal. Therefore the simple maximum likelihood estimation approach is sufficient here. If the likelihood hyper-surface was more complicated one could use the expectation-maximisation algorithm.
%\end{remark}


%% PROFILE LIKELIHOODS %%
%% ~ even mixture = multimodal
%\begin{figure}[p]
%\centering
%\includegraphics[width =\textwidth , height=11cm]{profile_like_plot1}
%\caption{Profile likelihood plots for CFG mixture model.}
%\label{profile_like_plot1}
%\end{figure}


%% ~0 Gumbel lambda = unimodal
%\begin{figure}[p]
%\centering
%\includegraphics[width =\textwidth , height=11cm]{profile_like_plot2}
%\caption{Profile likelihood plots for CFG mixture model.}
%\label{profile_like_plot2}
%\end{figure}



\FloatBarrier



==> (Matthew_Ames)_Innovations_in_Risk_Management/Introduction_GWP_26_Feb_2014.tex <==
\section{Currency Carry Trade and Uncovered Interest Rate Parity}

One of the most robust puzzles in finance still to be satisfactorily explained is the uncovered interest rate parity puzzle and the associated excess average returns of currency carry trade strategies. Such trading strategies are popular approaches which involve constructing portfolios by selling low interest rate currencies in order to buy higher interest rate currencies, thus profiting from the interest rate differentials. The presence of such profit opportunities, pointed out by \cite{Hansen1980,Fama1984,backus2001affine} and more recently by \cite{Lustig2007,Brunnermeier2008,burnside2011peso,christiansen2011time,Lustig2011,Menkhoff2012}, violates the fundamental relationship of uncovered interest rate parity (UIP). The UIP refers to the parity condition in which exposure to foreign exchange risk, with unanticipated changes in exchange rates, is uninhibited and therefore if one assumes rational risk-neutral investors, then changes in the exchange rates should offset the potential to profit from the interest rate differentials between high interest rate (investment) currencies and low interest rate (funding) currencies.
We can more formally write this relation by assuming that the forward price, $F_{t}^{T}$, is a martingale under the risk neutral probability $\mathbb{Q}$ (\cite{musiela2011martingale}): 
\begin{align}
E_{\mathbb{Q}}\Bigg[\frac{S_{T}}{S_{t}}\Bigg|\mathcal{F}_{t}\Bigg]=\frac{F_{t}^{T}}{S_{t}}=e^{(r_{t}-r_{t}^{\star})(T-t)}. \label{UIP}
\end{align}
The UIP Equation~(\ref{UIP}) thus states that under the risk neutral probability the expected variation of the exchange rate $S_{t}$ should equal the differential between the interest rate of the two associated countries, denoted by respectively $r_{t}$ and $r_{t}^{\star}$. The currency carry trade strategy investigated in this paper aims at exploiting violations of the UIP relation by investing a certain amount in a basket of high interest rate currencies (the long basket) while funding it through a basket of low interest rate currencies (the short basket).  When the UIP holds, then given foreign exchange market equilibrium, no profit should arise on average from this strategy; however such opportunities are routinely observed and exploited by large volume trading strategies.

In this paper we build on the existing literature by studying a stochastic feature of the joint tail behaviours of the currencies within each of the long and the short baskets, which form the carry trade. We aim to explore to what extent one can attribute the excess average returns with regard to compensation for exposure to tail risk, for example either dramatic depreciations in the value of the high interest rate currencies or dramatic appreciations in the value of the low interest rate currencies in times of high market volatility.

We postulate that such analyses should also benefit from consideration not only of the marginal behaviours of the processes under study, in this case the exchange rates of currencies in a portfolio, but also a rigorous analysis of the joint dependence features of such relationships. We investigate such joint relationships in light of the UIP condition. To achieve this, we study the probability of joint extreme movements in the funding and investment currency baskets and interpret these extremal tail probabilities as relative risk exposures of adverse and beneficial joint currency movements which would affect the portfolio returns. This allows us to obtain a relative contribution to the exposure of the portfolio profit decomposed in terms of the downside and upside risks that are contributed from such tail dependence features in each currency basket. We argue that the analysis of the carry trade is better informed by jointly modelling the multivariate behaviour of the marginal processes of currency baskets accounting for potential multivariate extremes, whilst still incorporating heavy-tailed relationships studied in marginal processes.

% To achieve the accurate modelling of the potentially complex multivariate dependence features the statistical models considered should be sufficiently flexible to accommodate a variety of potential tail dependence relationships. In this regard we consider two flexible families of mixture copula models comprised of members of the Archimedean copula family as well as the outer-power Clayton copula family, all of which admit different degrees of asymmetric upper and lower tail dependence.

%We are thus proposing in this manuscript, to explore the highly leveraged opportunities in currency carry trades that arise due to violation of the UIP. However, we conjecture that if the assessment of the risk associated with such trading strategies was modified to adequately take into account the potential for joint catastrophic risk events accounting for the non-trivial probabilities of joint adverse movements in currency exchange rates, then such strategies may not seem so profitable relative to the risk borne by the investor. 
%
%To perform this study we model the multivariate dependencies between exchange rate log returns using flexible families of mixture copula models comprised of members of the Archimedean copula family as well as the outer-power Clayton copula family. 
%This probabilistic approach allows us to express the joint distribution of the vectors of random variables, in our case vectors of exchange rate log-returns in each basket of currencies, as functions of each marginal distribution and the copula function itself.
We fit mixture copula models to vectors of daily exchange rate log returns between 1989 - 2014 for both the investment and funding currency baskets making up the carry trade portfolio. The method and the dataset considered for the construction of the respective funding and investing currencies baskets are thoroughly described in \cite{Ames2013}.
The currency compositions of the funding and investment baskets are varying daily over time as a function of the interest rate differential processes for each currency relative to the USD.

% However, there are several core currencies that consistently appear over time in the funding basket and likewise there are such currencies that appear in the investment basket consistently over time. We therefore take the model based tail dependence, upper and lower, for each basket (funding and investment) which represents the entire baskets financial risk exposure in a positive or negative direction, and we decompose each according to non-model dependent factors based on pairwise non-parametric tail dependence estimators obtained over time for one or more of these regularly incorporated currencies. This allows us to take the model based multivariate tail dependence and decompose it via a projection, which is model free, into the proportions of the positive and negative financial risk exposures for each basket according to its most important individual pairwise components. Thus we are able to interpret directly the influence on the risk attributed to the currency basket, either funding or investment, from individual currency pairs in the basket. Providing a clear understanding of the tail risk exposure decomposition by component of the funding and investment baskets.
  
Our analysis concludes that the appealing high return profile of a carry portfolio is not only compensating the tail thickness of each individual component probability distribution but also the fact that extreme returns tend to occur simultaneously and lead to a portfolio particularly sensitive to the risk of what is known as drawdown. Furthermore, we also demonstrate that high interest rate currency baskets and low interest rate currency baskets can display periods during which the tail dependence gets inverted, demonstrating when periods of construction of the aforementioned carry positions are being undertaken by investors.




==> (Matthew_Ames)_Innovations_in_Risk_Management/Joint_Tail_Risk_Exposure_GWP_26_02_2014_v1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Interpreting Tail Dependence as Financial Risk Exposure in Carry Trade Portfolios}
\label{joint_tail_risk_exposure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In order to fully understand the tail risks of joint exchange rate movements present when one invests in a carry trade strategy we can look at both the downside extremal tail exposure and the upside extremal tail exposure within the funding and investment baskets that comprise the carry portfolio. The downside tail exposure can be seen as the crash risk of the basket, i.e. the risk that one will suffer large joint losses from each of the currencies in the basket. These losses would be the result of joint appreciations of the currencies one is short in the low interest rate basket and/or joint depreciations of the currencies one is long in the high interest rate basket.

\begin{definition}[Downside Tail Risk Exposure in Carry Trade Portfolios]
\\Consider the funding currency (short) basket with $n$-exchange rates relative to base currency, on day $t$, with currency log-returns 
{\scriptsize{
$\smash{(X^{(1)}_t,X^{(2)}_t,\ldots,X^{(n)}_t)}$.}}
Then the downside tail exposure risk for the carry trade will be defined as the conditional probability of adverse currency movements in the short basket, corresponding to its upper tail dependence, given by
{\scriptsize{
\begin{equation}\label{EqnDown1}
\lambda_u^{(i)} (u) := \mathbb{P}\text{r}\left(X^{(i)}_t > F_i^{-1}(u)|X^{(1)}_t > F_1^{-1}(u),\ldots,X^{(i-1)}_t>F_{i-1}^{-1}(u), X^{(i+1)}_t>F_{i+1}^{-1}(u),\ldots,X^{(n)}_t>F_n^{-1}(u)\right)
\end{equation}
}}
for a currency of interest $i \in \left\{1,2,\ldots,n\right\}$. Conversely the downside tail exposure for the investment (long) basket with $n$ currencies will be defined as the conditional probability of adverse currency movement in the long basket, given by
{\scriptsize{
\begin{equation}\label{EqnDown2}
\lambda_l^{(i)}(u) := \mathbb{P}\text{r}\left(X^{(i)}_t < F_i^{-1}(u)|X^{(1)}_t < F_1^{-1}(u),\ldots,X^{(i-1)}_t < F_{i-1}^{-1}(u), X^{(i+1)}_t < F_{i+1}^{-1}(u),\ldots,X^{(n)}_t < F_n^{-1}(u)\right).
\end{equation}
}}
In general then a basket's upside or downside risk exposure would be quantified by the probability of a loss (or gain) arising from an appreciation or depreciation jointly of magnitude $u$ and the dollar cost associated to a given loss/gain of this magnitude. The standard approach in economics would be to associate say a linear cost function in $u$ to such a probability of loss to get say the downside risk exposure in dollars according to $E(u) = C_u({F_{X_t^{(i)}}(u)}) \times \lambda_u(u)$, which will be a function of the level $u$. As $\lambda_u$ becomes independent of the marginals, i.e. as $u \rightarrow 0$ or $u \rightarrow 1$, $C$ also becomes independent of the marginals.
\end{definition}

Conversely, we will also define the upside tail exposure that will contribute to profitable returns in the carry trade strategy when extreme movements that are in favour of the carry position held. These would correspond to precisely the probabilities discussed above applied in the opposite direction. That is the upside risk exposure in the funding (short) basket is given by Equation~(\ref{EqnDown1}) and the upside risk exposure in the investment (long) basket is given by Equation~(\ref{EqnDown2}). That is the upside tail exposure of the carry trade strategy is defined to be the risk that one will earn large joint profits from each of the currencies in the basket. These profits would be the result of joint depreciations of the currencies one is short in the low interest rate basket and/or joint appreciations of the currencies one is long in the high interest rate basket. 

\begin{rems} In a basket with $n$ currencies, $n \geq 2$, if one considers capturing the upside and downside financial risk exposures from a model based calculation of these extreme probabilities then
%\begin{enumerate}
%
if the parametric model is exchangeable, such as an Archimedean copula, then swapping currency $i$ in Equation (\ref{EqnDown1}) and Equation (\ref{EqnDown2}) with another currency from the basket, say $j$ will not alter the downside or upside risk exposures. If they are not exchangeable then one can consider upside and downside risks for each individual currency in the carry trade portfolio.

%
%\item{In popular models such as the Archimedean copula, the choice of joint upper tail exposure obtained by instead taking limits of multivariate conditional extreme probabilities for say some $1<r<n$ given by $\mathbb{P}\text{r}\left(\bm{X}^{(1:r)}_t|\bm{X}^{(n-r+1:n)}_t\right)$ will be in the limit of the upper or lower extremes, simply a scaled version of the result obtained in Equations \ref{EqnDown1} or \ref{EqnDown2}.
%}
%
%\end{enumerate}
\end{rems}

We thus consider these tail upside and downside exposures of the carry trade strategy as features that can show that even though average profits may be made from the violation of UIP, it comes at significant tail exposure. 
%One may consider parametric or non-parametric estimators in order to quantify these extreme risk exposures. In statistics if one takes values of $u$ at an extreme level such as $u \uparrow 1$ or $u \downarrow 0$ then these limiting $\lambda_u(u)$ and $\lambda_l(u)$ given by conditional probabilities are known as upper and lower tail dependence coefficients and they can be obtained from the copula model parameters directly in many cases.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Quantifying Upside and Downside Risk of the Carry Trade via Tail Dependence}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%
%% Tail Dependence
%%\section{Joint Tail Exposure in the Carry Trade via Extremal Tail Dependence Coefficient}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Interpreting Tail Dependence as Financial Risk Exposure in Carry Trade Portfolios}
%\label{joint_tail_risk_exposure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%In order to fully understand the tail risks of joint exchange rate movements present when one invests in a carry trade strategy we can look at both the downside extremal tail exposure and the upside extremal tail exposure within the funding and investment baskets that comprise the carry portfolio. The downside tail exposure can be seen as the crash risk of the basket, i.e. the risk that one will suffer large joint losses from each of the currencies in the basket. These losses would be the result of joint appreciations of the currencies one is short in the low interest rate basket and/or joint depreciations of the currencies one is long in the high interest rate basket.
%
%\begin{defi}[Downside Tail Risk Exposure in Carry Trade Portfolios]
%Consider the funding currency (short) basket with $n$-exchange rates relative to base currency, on day $t$, with currency log-returns $\left(X^{(1)}_t,X^{(2)}_t,\ldots,X^{(n)}_t\right)$. Then the downside tail exposure risk for the carry trade will be defined as the conditional probability of adverse currency movements in the short basket, given by
%{\small{
%\begin{equation}\label{EqnDown1}
% \mathbb{P}\text{r}\left(X^{(i)}_t > F^{-1}(u)|X^{(1)}_t > F^{-1}(u),\ldots,X^{(i-1)}_t>F^{-1}(u), X^{(i+1)}_t>F^{-1}(u),\ldots,X^{(n)}_t>F^{-1}(u)\right)
%\end{equation}
%}}
%for an currency of interest $i \in \left\{1,2,\ldots,n\right\}$. Conversely the downside tail exposure for the investment basket (long) basket with n currencies will be defined by the conditional probability of adverse currency movement in the long basket, given by
%{\small{
%\begin{equation}\label{EqnDown2}
%\mathbb{P}\text{r}\left(X^{(i)}_t < F^{-1}(u)|X^{(1)}_t < F^{-1}(u),\ldots,X^{(i-1)}_t < F^{-1}(u), X^{(i+1)}_t < F^{-1}(u),\ldots,X^{(n)}_t < F^{-1}(u)\right)
%\end{equation}
%}}
%\end{defi}
%
%Conversely we will also define the upside tail exposure that will contribute to profitable returns in the carry trade strategy when extreme movements are in favour of the carry position held are observed. These would correspond to precisely the probabilities discussed above applied in the opposite direction. That is the upside risk exposure in the funding (short) basket is given by Equation \ref{EqnDown2} and the upside risk exposure in the investment (long) basket is given by Equation \ref{EqnDown1}. That is the upside tail exposure is defined to be the risk that one will earn large joint profits from each of the currencies in the basket. These profits would be the result of joint depreciations of the currencies one is short in the low interest rate basket and/or joint appreciations of the currencies one is long in the high interest rate basket. 
%
%\begin{rems} In a basket with $n$ currencies $n \geq 2$ if one considers capturing the upside and downside financial risk exposures from a model based calculation of these extreme probabilities then two things should be noted:
%\begin{enumerate}
%%
%\item{If the parametric model is exchangeable, such as an Archimedean copula, then swapping currency $i$ in Equation \ref{EqnDown1} and Equation \ref{EqnDown2} with another currency from the basket, say $j$ will not alter the downside or upside risk exposures. If they are not exchangeable then one can consider upside and downside risks for each individual currency in the carry trade portfolio.
%}
%%
%\item{In popular models such as the Archimedean copula, the choice of joint upper tail exposure obtained by instead taking limits of multivariate conditional extreme probabilities for say some $1<r<n$ given by $\mathbb{P}\text{r}\left(\bm{X}^{(1:r)}_t|\bm{X}^{(n-r+1:n)}_t\right)$ will be in the limit of the upper or lower extremes, simply a scaled version of the result obtained in Equations \ref{EqnDown1} or \ref{EqnDown2}.
%}
%%
%\end{enumerate}
%\end{rems}
%
%We thus consider these tail upside and downside exposures as features that can show that even though average profits may be made from the violation of UIP, it comes at significant tail exposure. One may consider parametric or non-parametric estimators in order to quantify these extreme risk exposures. In statistics if one takes values of the threshold level $u$, that we consider the upside or downside risk with respect to, at an extreme level such as $u \uparrow 1$ or $u \downarrow 0$ then these limiting conditional probabilities are known as upper and lower tail dependence coefficients and they can be obtained from the copula model parameters directly in many cases.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Quantifying Upside and Downside Risk via Tail Dependence}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We can formalise the notion of the dependence behaviour in the extremes of the multivariate distribution through the concept of tail dependence, limiting behaviour of Equations (\ref{EqnDown1}) and (\ref{EqnDown2}), as $u \uparrow 1$ and $u \downarrow 0$ asymptotically.
% The tail dependence is defined as the conditional probability that a random vector exceeds a certain threshold given that the remaining components of the random vector in the joint distribution has exceeded this threshold. In the context of the applications we consider in this paper, this allows us to examine the probability that any sub-vector of the log return forward exchange rates for the basket of currencies will exceed a certain threshold given that the log return forward exchange rates for the remaining currencies in the basket have exceeded this threshold, in particular thresholds that are placing an interest in the tails of the multivariate distribution. 
The interpretation of such quantities is then directly relevant to assessing the chance of large adverse movements in multiple currencies which could potentially increase the risk associated with currency carry trade strategies significantly, compared to risk measures which only consider the marginal behaviour in each individual currency. 
Under certain statistical dependence models these extreme upside and downside tail exposures can be obtained analytically. we develop a flexible copula mixture example that has such properties below.



%, however this occasionally varies across the time period considered from a minimum of 2 up to a maximum of 6. Hence, there is no need for more complex copula structures such as vines since the dimension is relatively low.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% NOW SECTION 3 on COPULAS %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Generalised Archimedean Copula Models for Currency Exchange Rate Baskets}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Copula Model Based Parametric Estimator}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In order to study the joint tail dependence in the investment or funding basket we consider an overall tail dependence analysis which is parametric model based, obtained by using flexible mixtures of Archimedean copula components. Such a model approach is reasonable since typically the number of currencies in each of the long basket (investment currencies) and the short basket (funding currencies) is 4 or 5.

%As noted in the previous section we develop flexible mixture Archimedean copula models for the currency baskets. 
In addition these models have the advantage that they produce asymmetric dependence relationships in the upper tails and the lower tails in the multivariate model.
%In addition we can perform a type of model selection purely by incorporating into the estimation the mixture weights associated with each dependence hypothesis obtained from each mixture component. 
We consider three models; two Archimedean mixture models and one outer power transformed Clayton copula. The mixture models considered are the Clayton-Gumbel mixture and the Clayton-Frank-Gumbel mixture, where the Frank component allows for periods of no tail dependence within the basket as well as negative dependence. We fit these copula models to each of the long and short baskets separately.

\begin{definition}[Mixture Copula] 
A mixture copula is a linear weighted combination of copulae of the form:
\begin{equation}
C_M(\mathbf{u}; \mathbf{\theta}) = \sum_{i=1}^N \lambda_i C_i ({\bf u};{\bf \theta_i}),		%% CHANGE TO \Theta
\end{equation}
where  $0 \leq \lambda_i \leq 1 \;\; \forall i \in \{1, ..., N\}$ and $\sum_{i=1}^N \lambda_i = 1$.
\end{definition}

%Thus we can combine a copula with lower tail dependence, a copula with positive or negative dependence and a copula with upper tail dependence to produce a more flexible copula capable of modelling the multivariate log returns of forward exchange rates of a basket of currencies. 

%Since we consider Archimedean copula mixture components, we next recall the definition of the generator. A function $\psi$ is said to generate an Archimedean copula if it satisfies the properties in Definition \ref{archm_gen}.

%% Archimedean generator
%\begin{definition}[Archimedean Generator]
%An Archimedean generator is a continuous, decreasing function $\psi:[0, \infty) \rightarrow [0, 1]$ which satisfies the following conditions:
%\begin{enumerate}
%\item $\psi(0) = 1$,
%\item $\psi(\infty) = lim_{t \rightarrow \infty} \psi(t) = 0$,
%\item $\psi$ is strictly decreasing on $[0, inf\{t: \psi(t) = 0\}]$
%\end{enumerate}
%\label{archm_gen}
%\end{definition}

\begin{definition}[Archimedean Copula]
A d-dimensional copula C is called Archim- edean if it can be represented by the form:
\begin{equation}
C({\bf u}) = \psi \{\psi^{-1}(u_1) + \cdots + \psi^{-1}(u_d)\} = \psi \{t({\bf u}) \} \;\;\;\; \forall {\bf u} = \{u_1, \ldots, u_d\} \in [0, 1]^d ,
\label{eq:archimedean_copula}
\end{equation}
where $\psi$ is an Archimedean generator satisfying the conditions given in \cite{McNeil2009}. $\psi ^{-1}:[0, 1] \rightarrow [0, \infty)$ is the inverse generator with $\psi^{-1}(0) = \mbox{inf}\{t: \psi(t) = 0\}$.
\end{definition}

%One can then obtain formulas for computing the copula densities, of relevance to parameter estimation under a maximum likelihood approach.
% We can see from Equation~(\ref{eq:density}) that we are required to compute high dimensional derivatives of a composite function. In order to achieve this we utilise a specific multivariate chain rule result widely known as the Fa\`{a} di Bruno's Formula, see \cite{faa1857note} and discussions in\cite{constantine1996multivariate}. % and \cite{roman1980formula}. 

%\begin{definition}[Archimedean Copula Density]
%\cite{mcneil2009} prove that an Archimedean copula C admits a density c if and only if $\psi^{(d-1)}$ exists and is absolutely continuous on $(0, \infty)$. When this condition is satisfied, the copula density c is given by
%\begin{equation}
%c({\bf u})\;\; = \;\; \frac{ \partial^d C(u_1, \ldots , u_d)}{\partial u_1 \ldots \partial u_d} \;\;
%= \;\;\ \psi^{(d)} \{t({\bf u})\} \prod_{j=1}^d (\psi^{-1})'(u_j) \;\; , \;\;\;\; {\bf u} \in (0, 1)^d
%\label{eq:density}
%\end{equation}
%\end{definition}

In the following section we consider two stages to estimate the multivariate basket returns, firstly the estimation of suitable heavy tailed marginal models for the currency exchange rates (relative to USD), followed by the estimation of the dependence structure of the multivariate model composed of multiple exchange rates in currency baskets for long and short positions. 
%To achieve this we consider a copula model framework where we utilise the well-known result of Sklar's theorem (see \cite{Nelsen2006}) as it allows one to separate the multivariate distribution into its marginal distributions and the dependence structure between the margins known as a copula distribution, which is unique for continuous marginal models.

%This result demonstrates how copula models therefore provide a mechanism to model the marginal behaviour of each currency and then separately to focus on developing hypotheses regarding the possible dependence structures between the log returns of the forward exchange rates of the currencies in the baskets, which can be tested through parametrization of a model via a copula and then a process of model selection.






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% End of OLD SECTION 3 on COPULAS %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







%There are many possible copula models that could be considered in the modelling of the multivariate dependence features of the currency baskets.  Previously in the exchange rate modelling literature \cite{patton2006modelling} considered a symmetrized Joe-Clayton copula in order to capture the asymmetric dependence structure between the Deutsche mark and the yen. The author demonstrated the time-varying nature of the dependence, noting that the mark-dollar and yen-dollar exchange rates were more correlated when they were depreciating against the dollar than when they were appreciating. A flexible time-varying copula model is introduced by \cite{dias2010modeling} using the Fisher information to specify the dynamic correlation. The authors find a significantly time-varying correlation between Euro/US dollar and Yen/US dollar, dependent on the past return realizations.The intention of this analysis was to work with models that have well understood tail dependence features and are relatively parsimonious with regard to the number of parameters specifying the copula and the resulting tail dependence.

Once the parametric Archimedean mixture copula model has been fitted to a basket of currencies, it is possible to obtain the upper and lower tail dependence coefficients, via closed form expressions for the class of mixture copula models and outer-power transform models we consider. The tail dependence expressions for many common bivariate copulae can be found in \cite{Nelsen2006}. This concept was recently extended to the multivariate setting by \cite{de2012multivariate}.
% Now one may accurately interpret the tail dependence present between sub-vector partitions of the multivariate random vector of currency exchange rates in either basket with regard to joint tail dependence behaviours. 

\begin{definition}[Generalized Archimedean Tail Dependence Coefficient] 
Let $X = (X_1,..., X_n)^T$ be an n-dimensional random vector with distribution \newline $C(F_1(X_1), \ldots, F_n(X_n))$, where $C$ is an Archimedean copula and $F_1, ..., F_n$ are the marginal distributions. The coefficients of upper and lower tail dependence are defined respectively as:
\small{
% upper
\begin{equation}
\begin{aligned}
\lambda_u^{1,...,h|h+1,...,n} &= \lim_{u \rightarrow 1-} P\left( X_1 > F_1^{-1}(u),...,X_h > F_h^{-1}(u) | X_{h+1} > F_{h+1}^{-1}(u), ..., X_n > F_n^{-1}(u) \right) \\
&= \lim_{t \rightarrow 0^+} \frac{\sum_{i=1}^d \left( \binom{d}{d-i} i (-1)^{i} \left[ \psi^{'}  (it) \right] \right) }{\sum_{i=1}^{n-h} \left( \binom{n-h}{n-h-i} i (-1)^i \left[ \psi^{'} (it) \right] \right)} \;\;\;\; ,
\end{aligned}
\label{eq:archmuppertd}
\end{equation}}
% lower
\begin{equation}
\begin{aligned}
\lambda_l^{1,...,h|h+1,...,n} &= \lim_{u \rightarrow 0+} P \left( X_1 < F_1^{-1}(u),...,X_h < F_h^{-1}(u) | X_{h+1} < F_{h+1}^{-1}(u), ..., X_n < F_n^{-1}(u) \right) \\
&= \lim_{t \rightarrow \infty} \frac{n}{n-h} \frac{\psi^{'} (nt)}{\psi^{'} ((n-h)t)}
\end{aligned}
\label{eq:archmlowertd}
\end{equation}
%\end{definition}
\normalsize
for the model dependence function `generator' $\psi(\cdot)$ and its inverse function.
\end{definition}

%\begin{definition}[Generalized Archimedean Lower Tail Dependence Coefficient] 
%Let $X = (X_1,..., X_n)^T$ be an n-dimensional random vector with distribution function $C(F_1(X_1), \ldots, F_n(X_n))$, where C is an Archimedean copula and $F_1, ..., F_n$ are the marginal distributions. The coefficient of lower tail dependence is defined as:
%\small
%\begin{equation}
%\begin{aligned}
%\lambda_l^{1,...,h|h+1,...,n} &= \lim_{\nu \rightarrow 0+} P \left( X_1 < F_1^{-1}(\nu),...,X_h < F_h^{-1}(\nu) | X_{h+1} < F_{h+1}^{-1}(\nu), ..., X_n < F_n^{-1}(\nu) \right) \\
%&= \lim_{t \rightarrow \infty} \frac{n}{n-h} \frac{\psi^{'} (nt)}{\psi^{'} ((n-h)t)}
%\end{aligned}
%\label{eq:archmlowertd}
%\end{equation}
%\end{definition}

%\begin{rems}[Computing Numerical Limits for Upper Tail Dependence]
%In order to evaluate the expression~(\ref{eq:archmuppertd}) above for Archimedean copula generators is was necessary to use an iterative method of halves whereby $u$ was taken increasingly close to the limit of 1 until convergence of the estimate or numerical underflow was observed.
%\end{rems}

In \cite{de2012multivariate} the analogous form of the generalized multivariate upper and lower tail dependence coefficients for outer-power transformed Clayton copula models is provided.
%\begin{definition}[Outer Power Clayton Copula]
%The outer power Clayton copula model with asymmetric upper and lower tail dependence involves a generator given by $\psi(t) = (1+t^{1/\beta})^{-1/\rho}$ and its inverse $\psi^{-1}(t) = (t^{-\rho} + 1)^{\beta}$ and tail dependence given by
%\begin{equation} \label{OpCTD}
%\begin{split}
%\lambda_u^{1,...,h|h+1,...,n} & = \frac{\sum_{i=1}^n \left( \binom{n}{n-i} (-1)^{i} i^{1/ \beta} \right) }{\sum_{i=1}^{n-h} \left( \binom{n-h}{n-h-i} (-1)^i i^{1/ \beta} \right)} \\
%\lambda_l^{1,...,h|h+1,...,n} & =  \left(\frac{n}{n-h}\right)^{-1/(\beta \rho)}
%\end{split}
%\end{equation}
%\end{definition}
%%\lambda_l^{1,...,h|h+1,...,n} 
The derivation of Equations (\ref{eq:archmuppertd}) and (\ref{eq:archmlowertd}) for the outer power case follows from \cite{feller1971}, i.e. the composition of a completely monotone function with a non-negative function that has a completely monotone derivative is again completely monotone. 
%Such copula model transforms were also studied in \cite{nelsen1997}, where they are referred to as a beta family associated with the inverse generator $\psi^{-1}$. 
The densities for the outer power Clayton copula can be found in \cite{Ames2013}. % and can be calculated using equation (\ref{eq:density}).

In the above definitions of model based parametric upper and lower tail dependence one gets the estimates of joint extreme deviations in the whole currency basket. It will often be useful in practice to understand which pairs of currencies within a given currency basket contribute significantly to the downside or upside risks of the overall currency basket. In the class of Archimedean based mixtures we consider, the feature of exchangeability precludes decompositions of the total basket downside and upside risks into individual currency specific components. To be precise we aim to perform a decomposition of say the downside risk of the funding basket into contributions from each pair of currencies in the basket, we will do this is achieved via a simple linear projection onto particular subsets of currencies in the portfolio that are of interest, which leads for example to the following expression:
\begin{equation}
\mathbb{E}\left[\left.\hat  \lambda_u^{i|1,2,...,i-1,i+1,...,n} \right| \hat\lambda_u^{2|1}, \hat\lambda_u^{3|1}, \hat\lambda_u^{3|2},\ldots, \hat\lambda_u^{n|n-1}\right] = \alpha_0 + \sum_{i \neq j}^n \alpha_{ij}\hat\lambda_u^{i|j}, 
\end{equation}
where $\hat\lambda_u^{i|1,2,...,i-1,i+1,...,n}$ is a random variable since it is based on parameters of the mixture copula model which are themselves functions of the data and therefore random variables. Such a simple linear projection will then allow one to interpret directly the marginal linear contributions to the upside or downside risk exposure of the basket obtained from the model, according to particular pairs of currencies in the basket by considering the coefficients $\alpha_{ij}$, i.e. the projection weights. To perform this analysis we need estimates of the pairwise tail dependence in the upside and downside risk exposures $\hat\lambda_u^{i|j}$ and $\hat\lambda_l^{i|j}$ for each pair of currencies $i,j\in \left\{1,2,\ldots,n\right\}$. We obtain this through non-parametric (model-free) estimators, see \cite{Cruz2013}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Non-Parametric Estimator}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%The respective upper and lower pairwise tail dependencies within an n-dimensional Archimedean copula are necessarily equal due to the construction of the model. However, in reality it may not be true, for example that each pair of currencies within the high interest rate basket has the same upper tail dependence. Thus, it is informative to analyse the breakdown of the overall tail dependence within a basket by examining the tail dependence between each of the pairs. In order to achieve this and as a comparison to the tail dependence coefficients observed using the various parametric copula models, we used the following non-parametric estimator of upper tail dependence and the corresponding lower tail dependence, see \cite{Cruz2013}.% and \cite{NPTD_paper_from_IK}:

\begin{definition}Non-Parametric Pairwise Estimator of Upper Tail Dependence (Extreme Exposure) \\
\begin{equation}
\hat \lambda_u = 2 - \mbox{min} \left[2 \hspace{2mm}, \hspace{2mm} \frac{\mbox{log} \, \hat C_n \left( \frac{n - k}{n}, \frac{n - k}{n} \right)}{\mbox{log} (\frac{n - k}{n})} \right] \hspace{3mm} \hspace{3mm} k = {1,2, \ldots n-1},
\label{eq:nptd}
\end{equation}
where $\hat C_n \left( u_1, u_2 \right) = \frac{1}{n} \sum\limits_{i=1}^n \mathbf{1} \left( \frac{R_{1i}}{n} \leq u_1 , \frac{R_{2i}}{n} \leq u_2 \right)$
and $R_{ji}$ is the rank of the variable in its marginal dimension that makes up the pseudo data.
\end{definition}

In order to form a robust estimator of the upper tail dependence a median of the estimates obtained from setting $k$ as the $1^{st}, 2^{nd}, \ldots, 20^{th}$ percentile values was used. Similarly, $k$ was set to the $80^{th}, 81^{st}, \ldots, 99^{th}$ percentiles for the lower tail dependence.


==> (Matthew_Ames)_Innovations_in_Risk_Management/Results_GWP_27_Feb_2014_v1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Results and Discussion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%In this section we present a detailed analysis of the estimation of the marginal distributional models and the mixture copula models for both the high interest rate basket and the low interest rate basket. 
%Firstly, we investigate the goodness-of-fit for the marginal distributions of the exchange rate log-returns for the 34 currencies and then the goodness-of-fit for the various copula models considered. Following this, we interpret the time-varying dependence characteristics of the fitted copula models to the high and low interest rate baskets. 

In order to model the marginal exchange rate log-returns we considered two approaches. Firstly, we fit Log Generalised Gamma models to each of the 34 currencies considered in the analysis, updating the fits for every trading day based on a 6 month sliding window. A time series approach was also considered to fit the marginals, as is popular in much of the recent copula literature, see for example \cite{brechmann2012risk}, using GARCH(1,1) models for the 6 month sliding data windows. In each case we are assuming approximate local stationarity over these short 6 month time frames.

A summary of the marginal model selection can be seen in Table~\ref{AIC_margins}, which shows the average AIC scores for the 4 most frequent currencies in the high interest rate and the low interest rate baskets over the data period. Whilst the AIC for the GARCH(1,1) model is consistently lower than the respective AIC for the Generalised Gamma, the standard errors are sufficiently large for there to be no clear favourite between the two models.


% table size and spaces
\renewcommand{\arraystretch}{1.5}
\setlength{\tabcolsep}{8pt}
%[INSERT TABLE OF AIC AVERAGES PER 5 YEARS FOR MOST FREQUENT CURRENCIES]

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}%[htbp]
  \centering
  \caption{Average AIC for the Generalized Gamma (GG) and the GARCH(1,1) for the four most frequent currencies in the high interest rate and the low interest rate baskets over the 2001 - 2014 data period split into 2 chunks, i.e. 6 years. Standard deviations are shown in parentheses. Similar performance was seen between 1989-2001.}
    \begin{tabular}{cccccc}
%    \toprule
%    \textbf{} & \textbf{} & \multicolumn{2}{c}{\textbf{89 - 95}} & \multicolumn{2}{c}{\textbf{95 - 01}} \\
%    \midrule
%    \textbf{} & \textbf{Currency} & \textbf{GG} & \textbf{GARCH} & \textbf{GG} & \textbf{GARCH} \\
%    \multirow{4}[0]{*}{\begin{sideways}Investment\end{sideways}} & \textbf{TRY} & \textbf{-} & \textbf{-} & 347.5 (14.0) & \textbf{325.4 (46.7)} \\
%          & \textbf{MXN} & \textbf{-} & \textbf{-} & 357.5 (6.5) & \textbf{342.5 (22.7)} \\
%          & \textbf{ZAR} & 359.3 (3.6) & \textbf{346.8 (16.1)} & 356.3 (7.6) & \textbf{335.5 (39.2)} \\
%          & \textbf{BRL} & \textbf{-} & \textbf{-} & 362.1 (0.6) & \textbf{344.1 (9.1)} \\
%          \midrule
%    \multirow{4}[0]{*}{\begin{sideways}Funding\end{sideways}} & \textbf{JPY} & 360.8 (3.7) & \textbf{354.4 (7.8)} & 361.2 (1.6) & \textbf{355.9 (7.3)} \\
%          & \textbf{CHF} & 361.0 (0.7) & \textbf{357.4 (5.2)} & 361.0 (1.3) & \textbf{358.3 (3.4)} \\
%          & \textbf{SGD} & 358.7 (5.2) & \textbf{348.7 (12.0)} & 360.0 (3.3) & \textbf{345.9 (13.6)} \\
%          & \textbf{TWD} & \textbf{-} & \textbf{-} & 350.0 (9.2) & \textbf{338.2 (17.1)} \\
%          \bottomrule
%          & \textbf{} &       &       &       &  \\
           \toprule
          & \textbf{} & \multicolumn{2}{c}{\textbf{01 - 07}} & \multicolumn{2}{c}{\textbf{07 - 14}} \\
           \midrule
          & \textbf{Currency} & \textbf{GG} & \textbf{GARCH} & \textbf{GG} & \textbf{GARCH} \\
    \multirow{4}[0]{*}{\begin{sideways}Investment\end{sideways}} & \textbf{TRY} & 356.9 (3.5) & \textbf{341.1 (21.7)} & 358.7 (3.0) & \textbf{349.1 (16.8)} \\
          & \textbf{MXN} & 360.0 (1.2) & \textbf{357.04 (3.8)} & 358.6 (4.0) & \textbf{344.5 (28.1)} \\
          & \textbf{ZAR} & 358.7 (3.0) & \textbf{353.5 (11.4)} & 358.0 (6.1) & \textbf{352.8 (12.2)} \\
          & \textbf{BRL} & 359.0 (2.8) & \textbf{341.6 (19.4)} & 360.0 (2.1) & \textbf{341.6 (23.2)} \\
          \midrule	
    \multirow{4}[0]{*}{\begin{sideways}Funding\end{sideways}} & \textbf{JPY} & 361.2 (0.9) & \textbf{356.5 (7.2)} & 356.9 (6.8) & \textbf{355.0 (7.0)} \\
          & \textbf{CHF} & 360.8 (1.4) & \textbf{359.1 (2.9)} & 358.6 (7.4) & \textbf{355.4 (8.8)} \\
          & \textbf{SGD} & 360.0 (2.7) & \textbf{356.8 (5.7)} & 360.0 (2.6) & \textbf{353.7 (7.5)} \\
          & \textbf{TWD} & 358.7 (6.2) & \textbf{347.0 (16.4)} & 359.1 (5.8) & \textbf{348.5 (13.2)} \\
    \bottomrule
    \end{tabular}%
  \label{AIC_margins}%
\end{table}%

However, when we consider the model selection of the copula in combination with the marginal model we observe lower AIC  scores for copula models fitted on the pseudo data resulting from using Generalised Gamma margins than using GARCH(1,1) margins. This is the case for all three copula models under consideration in the paper. Figure~\ref{CFG_GG_vs_GARCH_high_and_low} shows the AIC differences when using the Clayton-Frank-Gumbel copula in combination with the two choices of marginal for the high interest rate and the low interest rate basket respectively.
Over the entire data period the mean difference between the AIC scores for the CFG model with Generalised Gamma vs GARCH(1,1) marginals for the high interest rate basket is 12.3 and for the low interest rate basket is 3.6 in favour of the Generalised Gamma.

\begin{figure}%[p]
\centering
\includegraphics[width =\textwidth , height = 60mm]{figures/CFG_GG_vs_GARCH_high_and_low}
\caption{Comparison of AIC for Clayton-Frank-Gumbel model fit on the pseudo data resulting from Generalised Gamma vs GARCH(1,1) margins . The high interest rate basket is shown in the upper panel and the low interest rate basket is shown in the lower panel.}
\label{CFG_GG_vs_GARCH_high_and_low}
\end{figure}

Thus, it is clear that the Generalised Gamma model is the better model in our copula modelling context and so is used in the remainder of the analysis. We now consider the goodness-of-fit of the three copula models applied to the high interest rate basket and low interest rate basket pseudo data. We used a scoring via the AIC between the three component mixture CFG model versus the two component mixture CG model versus the two parameter OpC model. One could also use the Copula-Information-Criterion (CIC), see \cite{Gronneberg2010} for details. 

The results are presented for this comparison in Figure~\ref{CFG_GG_vs_CG_OpC_high_and_low}, which shows the differentials between AIC for CFG versus CG and CFG versus OpC for each of the high interest rate and the low interest rate currency baskets. We can see it is not unreasonable to consider the CFG model for this analysis, since over the entire data period the mean difference between the AIC scores for the CFG and the CG models for the high interest rate basket is 1.33 and for the low interest rate basket is 1.62 in favour of the CFG.

However, from Figure~\ref{CFG_GG_vs_CG_OpC_high_and_low} we can see that during the Credit crisis period the CFG model is performing much better.
The CFG copula model provides a much better fit when compared to the OpC model, as shown by the mean difference between the AIC scores of 9.58 for the high interest rate basket and 9.53 for the low interest rate basket. Similarly, the CFG model performs markedly better than the OpC model during the Credit crisis period.

\begin{figure}%[p]
\centering
\includegraphics[width =\textwidth , height = 60mm]{figures/CFG_GG_vs_CG_OpC_high_and_low}
\caption{Comparison of AIC for Clayton-Frank-Gumbel model with Clayton-Gumbel and Outer power Clayton models on high and low interest rate baskets with Generalised Gamma margins. The high interest rate basket is shown in the upper panel and the low interest rate basket is shown in the lower panel.}
\label{CFG_GG_vs_CG_OpC_high_and_low}
\end{figure}

%\begin{remark}
%Many fits gave a negligible weighting to the Frank component of the CFG copula, in particular during the first 10 years when we have only bivariate baskets. Thus, the AIC difference for those days can be seen in Figure~\ref{CFG_GG_vs_CG_OpC_high_and_low} to be very close to +4 = (2 $\times$ difference in number of parameters between CFG and CG copulae).
%\end{remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Tail Dependence Results}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Below we will examine the time-varying parameters of the maximum likelihood fits of this mixture CFG copula model. Here, we shall focus on the strength of dependence present in the currency baskets, given the particular copula structures in the mixture, which is considered as tail upside/downside exposure of a carry trade over time. Figure~\ref{CFG_OPC_VIX_high_TD} shows the time-varying upper and lower tail dependence, i.e. the extreme upside and downside risk exposures for the carry trade basket, present in the high interest rate basket under the CFG copula fit and the OpC copula fit. Similarly, Figure~\ref{CFG_OPC_VIX_low_TD} shows this for the low interest rate basket. 

\begin{remark}[Model Risk and its Influence on Upside and Downside Risk Exposure]
In fitting the OpC model, we note that independent of the strength of true tail dependence in the multivariate distribution, the upper tail dependence coefficient $\lambda_u$ for this model strictly increases with dimension very rapidly. Therefore, when fitting the OpC model, if the basket size becomes greater than bivariate, i.e. from 1999 onwards, the upper tail dependence estimates become very large (even for outer-power parameter values very close to $\beta=1$). This lack of flexibility in the OpC model only becomes apparent in baskets of dimension greater than 2, but is also evident in the AIC scores in Figure~\ref{CFG_GG_vs_CG_OpC_high_and_low}. Here we see an interesting interplay between the model risk associated to the dependence structure being fit and the resulting interpreted upside or downside financial risk exposures for the currency baskets.
\end{remark}

Focusing on the tail dependence estimate produced from the CFG copula fits we can see that there are indeed periods of heightened upper and lower tail dependence in the high interest rate and the low interest rate baskets. There is a noticeable increase in upper tail dependence in the high interest rate basket at times of global market volatility. Specifically, during late 2007, i.e. the global financial crisis, there is a sharp peak in upper tail dependence. Preceding this, there is an extended period of heightened lower tail dependence from 2004 to 2007, which could tie in with the building of the leveraged carry trade portfolio positions. This period of carry trade construction is also very noticeable in the low interest rate basket through the very high levels of upper tail dependence.

%% -------------- TD vs VIX -------------------- %%
% high
\begin{figure}%[p]
\centering
\includegraphics[width =\textwidth , height=80mm]{figures/CFG_OPC_VIX_high_TD2}
\caption{Comparison of Volatility Index (VIX) with upper and lower tail dependence of the high interest rate basket in the CFG copula and OpC copula. US NBER recession periods are represented by the shaded grey zones. Some key crisis dates across the time period are labelled.}
\label{CFG_OPC_VIX_high_TD}
\end{figure}

% low
\begin{figure}%[p]
\centering
\includegraphics[width =\textwidth , height=80mm]{figures/CFG_OPC_VIX_low_TD2}
\caption{Comparison of Volatility Index (VIX) with upper and lower tail dependence of the low interest rate basket in the CFG copula and OpC copula. US NBER recession periods are represented by the shaded grey zones. Some key crisis dates across the time period are labelled.}
\label{CFG_OPC_VIX_low_TD}
\end{figure}

We compare in Figures~\ref{CFG_OPC_VIX_high_TD} and \ref{CFG_OPC_VIX_low_TD} the tail dependence plotted against the VIX volatility index for the high interest rate basket and the low interest rate basket respectively for the period under investigation. The VIX is a popular measure of the implied volatility of S\&P 500 index options - often referred to as the \emph{fear index}. As such it is one measure of the market's expectations of stock market volatility over the next 30 days. We can clearly see here that in the high interest rate basket there are upper tail dependence peaks at times when there is an elevated VIX index, particularly post-crisis. However, we would not expect the two to match exactly since the VIX is not a direct measure of global FX volatility. We can thus conclude that investors' risk aversion clearly plays an important role in the tail behaviour. This conclusion corroborates recent literature regarding the skewness and the kurtosis features characterizing the currency carry trade portfolios \cite{Farhi2008,Brunnermeier2008, Menkhoff2012}.

\subsection{Pairwise Decomposition of Basket Tail Dependence}

In order to examine the contribution of each pair of currencies to the overall n-dimensional basket tail dependence we calculated the corresponding non-parametric pairwise tail dependencies for each pair of currencies. In Figure~\ref{crisis3_heatmap} we can see the average upper and lower non-parametric tail dependence for each pair of currencies during the Credit crisis, with the 3 currencies most frequently in the high interest rate and the low interest rate baskets labelled accordingly. The lower triangle represents the non-parametric pairwise lower tail dependence and the upper triangle represents the non-parametric pairwise upper tail dependence.

If one was trying to optimise their currency portfolio with respect to the tail risk exposures, i.e. to minimise negative tail risk exposure and maximise positive tail risk exposure, then one would sell short currencies with high upper tail dependence and low lower tail dependence whilst buying currencies with low upper tail dependence and high lower tail dependence.
%[INSERT MORE ANALYSIS HERE...]

% Credit Crisis
\begin{figure}%[p]
\centering
\includegraphics[width =\textwidth, height=75mm]{figures/crisis_3_hmBONE}	%
\caption{Heat map showing the strength of non-parametric tail dependence between each pair of currencies averaged over the Credit crisis period. Lower tail dependence is shown in the lower triangle and upper tail dependence is shown in the upper triangle. The 3 currencies most frequently in the high interest rate and the low interest rate baskets are labelled.}
\label{crisis3_heatmap}
\end{figure}

Similarly, in Figure~\ref{last_12_months_heatmap} we see the pairwise non-parametric tail dependencies averaged over the last 12 months (01/02/2013 to 29/01/2014). Comparing this heat map to the heat map during the Credit crisis (Figure~\ref{crisis3_heatmap}) we notice that in general there are lower values of tail dependence amongst the currency pairs.

%[INSERT MORE ANALYSIS HERE...]

% last 12 months heatmap
\begin{figure}%[p]
\centering
\includegraphics[width =\textwidth, height=75mm]{figures/last_12_months_hmBONE}
\caption{Heat map showing the strength of non-parametric tail dependence between each pair of currencies averaged over the last 12 months (01/02/2013 to 29/01/2014). Lower tail dependence is shown in the lower triangle and upper tail dependence is shown in the upper triangle. The 3 currencies most frequently in the high interest rate and the low interest rate baskets are labelled.}
\label{last_12_months_heatmap}
\end{figure}




%% REGRESSION


We performed linear regression of the pairwise non-parametric tail dependence on the respective basket tail dependence for the days on which the 3 currencies all appeared in the basket (224 out of 250 for the lower interest rate basket and 223 out of 250 for the high interest rate basket). The regression coefficients and $R^2$ values can be seen in Table~\ref{nptd_td_regression}. We can interpret this as the relative contribution of each of the 3 currency pairs to the overall basket tail dependence. We note that for the low interest rate lower tail dependence and for the high interest rate upper tail dependence there is a significant degree of cointegration between the currency pair covariates and hence we might be able to use a single covariate due to the presence of a common stochastic trend.

%[INSERT MORE ANALYSIS HERE...]


%[INSERT TABLE of Betas]
\setlength{\tabcolsep}{6pt}
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}%[htbp]
  \centering
  \caption{Pairwise non-parametric tail dependence regressed on respective basket tail dependence (standard errors are shown in parentheses). The 3 currencies most frequently in the respective baskets are used as independent variables.}
    \begin{tabular}{cccccc}
    \toprule
    \textbf{Low IR Basket } & \textbf{Constant} & \textbf{CHF JPY} & \textbf{CZK CHF} & \textbf{CZK JPY} & \textbf{$R^2$} \\
    \midrule
    \textbf{Upper TD} & 0.22 (0.01)  & 0.02 (0.03)  & 0.18 (0.02)  & 0.38 (0.05)  & 0.57 \\
    \textbf{Lower TD} & 0.71 (0.17)  & -0.62 (0.25) & -0.38 (0.26) & 0.23 (0.32)  & 0.28 \\
    \bottomrule
    \textbf{} &       &       &       &       &  \\
        \toprule
    \textbf{High IR Basket } & \textbf{Constant} & \textbf{EGP INR} & \textbf{UAH EGP} & \textbf{UAH INR} & \textbf{$R^2$} \\
        \midrule
    \textbf{Upper TD} & 0.07 (0.01)  & -0.06 (0.33) & 0.59 (0.08)  & 2.37 (0.42)  & 0.4 \\
    \textbf{Lower TD} & 0.1 (0.02)   & 0.56 (0.05)  & 0.44 (0.08)  & -0.4 (0.07)  & 0.44 \\
    \bottomrule
    \end{tabular}%
  \label{nptd_td_regression}%
\end{table}%









\subsection{Understanding the Tail Exposure associated with the Carry Trade and its Role in the UIP Puzzle}

%In the existing literature, the risks associated with the carry trade have been analysed from the marginal perspective or from an aggregated portfolio perspective, i.e. taking into account the mean, variance, skewness and kurtosis of portfolio returns, see \cite{Menkhoff2012,Lustig2011,Brunnermeier2008}. However, until now the tails in the dependence structure within each basket of the carry trade have been overlooked as an additional source of risk. It is important to note that in our paper we study the extremal tail exposure, not the intermediate tail risk (see \cite{hua2012strength,hua2012intermediate}), and hence we focus on the relative effect of the extreme exposures on portfolio returns. In order to have a better grasp of the risk globally associated to a currency carry trade portfolio, which is derived from the differential of interest rates, we propose to compare the relative tail exposure adjusted returns for the two components of such a portfolio, namely the high and the low interest rates baskets.

As was discussed in Section~\ref{joint_tail_risk_exposure}, the tail exposures associated with a currency carry trade strategy can be broken down into the upside and downside tail exposures within each of the long and short carry trade baskets.
%The downside tail exposure can be seen as the crash risk of the basket, i.e. the risk that one will suffer large joint losses from each of the currencies in the basket. These losses would be the result of joint appreciations of the currencies one is short in the low interest rate basket and/or joint depreciations of the currencies one is long in the high interest rate basket. The downside tail exposures are thus characterised by the conditional probabilities that one or more currencies in the long/short basket depreciates/appreciates beyond an extreme threshold given that the remaining currencies in the long/short basket depreciate/appreciate beyond this threshold.
%The upside tail exposure is the risk that one will earn large joint profits from each of the currencies in the basket. These profits would be the result of joint depreciations of the currencies one is short in the low interest rate basket and/or joint appreciations of the currencies one is long in the high interest rate basket. The upside tail exposures are thus characterised by the conditional probabilities that one or more currencies in the short/long basket depreciates/appreciates beyond an extreme threshold given that the remaining currencies in the short/long basket depreciate/appreciate beyond this threshold.
The downside relative exposure adjusted returns are obtained by multiplying the monthly portfolio returns by one minus the upper and the lower tail dependence present respectively in the high interest rate basket and the low interest rate basket at the corresponding dates. The upside relative exposure adjusted returns are obtained by multiplying the monthly portfolio returns by one plus the lower and upper tail dependence present respectively in the high interest rate basket and the low interest rate basket at the corresponding dates. Note that we refer to these as relative exposure adjustments only for the tail exposures since we do not quantify a market price per unit of tail risk. However, this is still informative as it shows a decomposition of the relative exposures from the long and short baskets with regard to extreme events.

As can be seen in Figure~\ref{risk_adj_Downside}, the relative adjustment to the absolute cumulative returns for each type of downside exposure is greatest for the low interest rate basket, except under the OpC model, but this is due to the very poor fit of this model to baskets containing more than 2 currencies which we see transfers to financial risk exposures. This is interesting because intuitively one would expect the high interest rate basket to be the largest source of tail exposure. However, one should be careful when interpreting this plot, since we are looking at the extremal tail exposure. The analysis may change if one considered the intermediate tail risk exposure, where the marginal effects become significant.
Similarly, Figure~\ref{risk_adj_Upside} shows the relative adjustment to the absolute cumulative returns for each type of upside exposure is greatest for the low interest rate basket. The same interpretation as for the downside relative exposure adjustments can be made here for upside relative exposure adjustments.






%% Risk Adjusted Plots

%[ADD in OpC to this plot]


% Downside Risk adjusted HML returns
\begin{figure}%[p]
\centering
\includegraphics[width =\textwidth , height=75mm]{figures/downside_risk_adj_returns}
\caption{Cumulative log returns of the carry trade portfolio (HML = High interest rate basket Minus Low interest rate basket). Downside exposure adjusted cumulative log returns using upper/lower tail dependence in the high/low interest rate basket for the CFG copula and the OpC copula are shown for comparison.}
\label{risk_adj_Downside}
\end{figure}


% Upside Risk adjusted HML returns
\begin{figure}%[p]
\centering
\includegraphics[width =\textwidth ,height=75mm]{figures/upside_risk_adj_returns}
\caption{Cumulative log returns of the carry trade portfolio (HML = High interest rate basket Minus Low interest rate basket). Upside exposure adjusted cumulative log returns using lower/upper tail dependence in the high/low interest rate basket for the CFG copula and the OpC copula are shown for comparison.}
\label{risk_adj_Upside}
\end{figure}

%\FloatBarrier

==> CopulaModels_GWP_26_Feb_2014_v1_0_0.tex <==
\section{Generalised Archimedean Copula Models for Currency Exchange Rate Baskets}

As noted in the previous section we develop flexible mixture Archimedean copula models for the currency baskets. Such models have the advantage that they produce asymmetric dependence relationships in the upper tails and the lower tails in the multivariate model.
In addition we can perform a type of model selection purely by incorporating into the estimation the mixture weights associated with each dependence hypothesis obtained from each mixture component. We consider three models; two Archimedean mixture models and one outer power transformed Clayton copula. The mixture models considered are the Clayton-Gumbel mixture and the Clayton-Frank-Gumbel mixture, where the Frank component allows for periods of no tail dependence within the basket as well as negative dependence. We fit these copula models to each of the long and short baskets separately. 

\begin{definition}[Mixture Copula] 
A mixture copula is a linear weighted combination of copulae of the form:
\begin{equation}
C_M(\mathbf{u}; \mathbf{\theta}) = \sum_{i=1}^N w_i C_i ({\bf u};{\bf \theta_i}) 		%% CHANGE TO \Theta
\end{equation}
where  $0 \leq w_i \leq 1 \;\; \forall i \in \{1, ..., N\}$ and $\sum_{i=1}^N w_i = 1$
\end{definition}

Thus we can combine a copula with lower tail dependence, a copula with positive or negative dependence and a copula with upper tail dependence to produce a more flexible copula capable of modelling the multivariate log returns of forward exchange rates of a basket of currencies. 

%Since we consider Archimedean copula mixture components, we next recall the definition of the generator. A function $\psi$ is said to generate an Archimedean copula if it satisfies the properties in Definition \ref{archm_gen}.

% Archimedean generator
\begin{definition}[Archimedean Generator]
An Archimedean generator is a continuous, decreasing function $\psi:[0, \infty) \rightarrow [0, 1]$ which satisfies the following conditions:
\begin{enumerate}
\item $\psi(0) = 1$,
\item $\psi(\infty) = lim_{t \rightarrow \infty} \psi(t) = 0$,
\item $\psi$ is strictly decreasing on $[0, inf\{t: \psi(t) = 0\}]$
\end{enumerate}
\label{archm_gen}
\end{definition}

\begin{definition}[Archimedean Copula]
A d-dimensional copula C is called Archim- edean if it can be represented as:
\begin{equation}
C({\bf u}) = \psi \{\psi^{-1}(u_1) + \cdots + \psi^{-1}(u_d)\} = \psi \{t({\bf u}) \} \;\;\;\; \forall {\bf u} \in [0, 1]^d
\label{eq:archimedean_copula}
\end{equation}
where $\psi$ is an Archimedean generator and $\psi ^{-1}:[0, 1] \rightarrow [0, \infty)$ is the inverse generator with $\psi^{-1}(0) = inf\{t: \psi(t) = 0\}$.
\end{definition}

One can then obtain formulas for computing the copula densities, of relevance to parameter estimation under a maximum likelihood approach. We can see from Equation~(\ref{eq:density}) that we are required to compute high dimensional derivatives of a composite function. In order to achieve this we utilise a specific multivariate chain rule result widely known as the Fa\`{a} di Bruno's Formula, see \cite{faa1857note} and discussions in for example \cite{constantine1996multivariate} and \cite{roman1980formula}. 

\begin{definition}[Archimedean Copula Density]
\cite{mcneil2009} prove that an Archimedean copula C admits a density c if and only if $\psi^{(d-1)}$ exists and is absolutely continuous on $(0, \infty)$. When this condition is satisfied, the copula density c is given by
\begin{equation}
c({\bf u})\;\; = \;\; \frac{ \partial^d C(u_1, \ldots , u_d)}{\partial u_1 \ldots \partial u_d} \;\;
= \;\;\ \psi^{(d)} \{t({\bf u})\} \prod_{j=1}^d (\psi^{-1})'(u_j) \;\; , \;\;\;\; {\bf u} \in (0, 1)^d
\label{eq:density}
\end{equation}
\end{definition}




